A Distributed Adaptive Algorithm for Non-Smooth Spatial Filtering Problems in Wireless Sensor Networks

A wireless sensor network often relies on a fusion center to process the data collected by each of its sensing nodes. Such an approach relies on the continuous transmission of raw data to the fusion center, which typically has a major impact on the sensors' battery life. To address this issue in the particular context of spatial filtering and signal fusion problems, we recently proposed the Distributed Adaptive Signal Fusion (DASF) algorithm, which distributively computes a spatial filter expressed as the solution of a smooth optimization problem involving the network-wide sensor signal statistics. In this work, we show that the DASF algorithm can be extended to compute the filters associated with a certain class of non-smooth optimization problems. This extension makes the addition of sparsity-inducing norms to the problem's cost function possible, allowing sensor selection to be performed in a distributed fashion, alongside the filtering task of interest, thereby further reducing the network's energy consumption. We provide a description of the algorithm, prove its convergence, and validate its performance and solution tracking capabilities with numerical experiments.

==> fc_procedure.tex <==
\begin{figure}
        \centering
\tikzstyle{node}=[circle,draw=none,fill=blue!20,minimum size=1.5em,inner sep=0pt]
\tikzstyle{updating}=[circle,draw=none,fill=red!40,minimum size=1.5em,inner sep=0pt]
\begin{tikzpicture}
        \node[updating] (k1) at (0,0) {$1$};
        \node[node] (k2) at (1.5,-1.5) {$2$};
        \node[node] (k3) at (0,-3) {$3$};
        \node[node] (k4) at (-1.5,-1.5) {$4$};

        \draw[-Latex] (k2) to[bend right] node[midway,above, sloped,
                align=center] {$\ly_2,\Al_2, \cB_2, \cC_2$} (k1);
        \draw[-Latex] (k3) to node[midway,above, sloped]
                {$\ly_3,\Al_3, \cB_3 \cC_3$} (k1);
        \draw[-Latex] (k4) to[bend left] node[midway,above, sloped]
                {$\ly_4,\Al_4, \cB_4,\cC_4$} (k1);

        \node[updating] (k1bis) at (5, 0) {$1$};
        \node[node] (k2bis) at (6.5,-1.5) {$2$};
        \node[node] (k3bis) at (5,-3) {$3$};
        \node[node] (k4bis) at (3.5,-1.5) {$4$};

        \draw[-Latex] (k1bis) to[bend left] node[midway,above, sloped,
                align=center] {$\lX_2^\star$} (k2bis);
        \draw[-Latex] (k1bis) to node[midway,above, sloped]
                {$\lX_3^\star$} (k3bis);
        \draw[-Latex] (k1bis) to[bend right] node[midway,above, sloped]
                {$\lX_4^\star$} (k4bis);

\end{tikzpicture}
\caption{Exchanged data in a fully-connected network at an iteration where node 1 is the updating node (iteration index omitted). Left: Data aggregation to
        the updating node $1$. Right: Filters
    update. Note that the exchange of $\A_k$, $\B_k$, $\C_k$ and $\X_k$ is
negligible compared to a batch of $N$ samples of $\bm{y}_k$.}
\label{fig:fc_procedure}
\end{figure}


==> inexactalg.tex <==
\section{Inexact Iterative Local Solver}
\label{sec:inexactalg}

\wip{General idea: consider local solver satisfying $M\norm{\X^{j}-\X^{j-1}}\leq
L(\X^{j-1})-L(\X^j)$. It ensures that it is also true for $i$ instead on $j$ by
summing and telsscroping. The consequence is that $X^i-X^{i-1}\to 0$ . We also
require that fixed points of local solver are local solutions (foxed point alg). }
\wip{Give exmaples of solver satisfying the conditions , ex. manifold solvers,
proximal gradient, monotone schemes?}

Algorithm \wip{ALG} is in practice not implementable, as it requires the
computation of an exact solution of \eqref{eq:local_eval} at each iteration,
which is in general not possible. In this section, we replace the abstract
solver computing the $\argmin$ by an inexact iterative local solver. Given some
$\X^i$, the inexact iterative local solver produces a sequence of iterates
$(\X^{i,j})_{j\in\mathbb{N}}$ such that 
\begin{enumerate}
        \item $\X^{i,0}=\X^{i}$,
        \item there is some $R<\infty$ such that $L(\X^{i,j})-L(\X^{i,j+1})\geq
                R\norm{\X^{i,j}-\X^{i,j+1}}$, and
        \item $\lim_{j\to\infty}\X^{i,j}$ is a stationary point of
                \eqref{eq:local_problem3}.
\end{enumerate}
\wip{Reference to Attouch on th econvergence of such algorithms for
semialgebraioc problems}

The inexact version of Algorithm \wip{ALG} simply consists in selecting 
\begin{equation}
        \X^{i+1}=\X^{i,N_i}
\end{equation}
with $N_i>0$.

\begin{theorem}
        \label{th:inexact}
        Let $(\X^i)_{i\in\mathbb{N}}$ be the sequence generated by Algorithm
        \wip{ALG} with inexact local solver. Then, $(\X^i)_{i\in\mathbb{N}}$
        converges to a stationary point of \eqref{eq:generic_problem}.
\end{theorem}
\begin{proof}
        We first notice that the sufficient decrease property of the local
        solver is inherited by the full algorithm. Indeed, for any $i$,
        \begin{equation}
        \sum_{j=1}^{N_i} L(\X^{i,j})-L(\X^{i,j+1}) \geq \sum_{j=1}^{N_i}
        R\norm{\X^{i,j}-\X^{i,j+1}},
\end{equation}
and thus, using the triangle inequality for the right sum, 
\begin{equation}
        L(\X^i)-L(\X^{i+1})\geq R\norm{\X^i-\X^{i+1}}.
\end{equation}
\wip{Comment on $R$}
As $L(\X^i)$ converges, it must be that $\norm{\X^i-\X^{i+1}}\to0$. This also
implies that $\lim_{i\to\infty}\norm{\X^{i,j}-\X^{i,j+1}}=0$ for any $j$ and
therefore 
\begin{equation}
        \lim_{i\to\infty}\lim_{j\to\infty}\X^{i,j}=\lim_{i\to\infty}\X^i=\X^\star
\end{equation}
is a stationary point of the local problem \eqref{eq:local_problem3}.
\wip{bevause of XI going to Xip1m, fixed point of one is fixed point of all can
apply previous theorem}

\end{proof}



==> node_selection.tex <==
\section{Node Selection in Multi-Task Networks}
\wip{SUMCOR??}


==> tree_branches.tex <==
\begin{figure}
    \centering
    \tikzstyle{place}=[circle,fill=blue!20, minimum size=0.8cm, scale=0.6, node distance=1.5cm]
    \tikzstyle{leaf}=[circle,fill=red!20, minimum size=0.8cm, scale=0.6, node distance=1.5cm]
    \tikzstyle{halo}=[circle, minimum size=1cm]
    \begin{tikzpicture}[use Hobby shortcut, scale=0.8]

        \node[place] (2) at (4, 0) {$k_2$};
        \node[leaf] (2a) [right of=2] {};
        \node[place] (2b) [above left of=2] {$q$};
        \node[leaf] (2c) [above right of=2] {};
        \node[leaf] (2bb) [above of=2b] {$k_1$};

        \path 
        (2) edge (2a)
        (2) edge (2b)
        (2) edge (2c)
        (2b) edge (2bb)
        ;


        \node[leaf] (3) at (1.5, 2) {};
        \node[place] (3a) [below of=3] {$k_3$};
        %\node[leaf] (3b) [above left of=3] {};
        %\node[leaf] (3c) [above right of=3] {};

        \path 
        (3) edge (3a)
        % (3) edge (3b)
        % (3) edge (3c)
        ;

        \node[place] (1c) [above left of=3a] {};
        \node[leaf] (1) at (-0.5, 0.5) {};
        \node[place] (1a) [above of=1] {};
        \node[leaf] (1b) [above left of=1] {};
        

        \path 
        (1c) edge (1a)
        (1) edge (1a)
        (1a) edge (1b)
        (1) edge (1a)
        ;

        \path (2b) edge (3a)
        (3a) edge (1c);

        \node[scale=0.7]  (label1) at (-0.7, 2.7) {$\mathcal{B}_{k_3q}$};
        \node[scale=0.7]  (label1) at (4.2, 2.5) {$\mathcal{B}_{k_1q}$};
        \node[scale=0.7]  (label1) at (2.7, 0) {$\mathcal{B}_{k_2q}$};

        \begin{pgfonlayer}{background}
            \node[halo, fill=orange!10, draw=orange] (2bbo) at (2bb) {};


            \node[halo] (2o) at (2) {};
            \node[halo] (2ao) at (2a) {}; 
            \node[halo] (2co) at (2c) {}; 
            \draw[fill=cyan!10, draw=cyan] (2o.west) to[closed, curve through={(2o.north) .. (2co.west) .. (2co.north) .. (2co.east) .. (2ao.east)} ] (2o.south);
        \end{pgfonlayer}

        % \begin{pgfonlayer}{background}
        %     \node[halo] (1o) at (1) {};
        %     \node[halo] (1ao) at (1a) {};
        %     \node[halo] (1bo) at (1b) {}; 

        %     \node[halo] (3bo) at (3b) {}; 
        %     \node[halo] (3co) at (3c) {};
        %     \node[halo] (3ao) at (3a) {};
        %     \node[halo] (3o) at (3) {}; 

        %     \draw[draw=green, fill=green!10] (1bo.north) to[closed, curve through={(1ao.north) .. (3bo.west) .. (3bo.north) .. (3co.east) .. (3o.east) .. (3ao.east) .. (3ao.south) .. (1o.south)} ] (1bo.west);
        % \end{pgfonlayer}

        \begin{pgfonlayer}{background}
            \node[halo] (1o) at (1) {};
            \node[halo] (1ao) at (1a) {};
            \node[halo] (1bo) at (1b) {}; 

            \node[halo] (3ao) at (3a) {};
            \node[halo] (3o) at (3) {}; 

            \draw[draw=green, fill=green!10] (1bo.north) to[closed, curve through={(1ao.north) .. (3o.east) .. (3ao.east) .. (3ao.south) .. (1o.south)} ] (1bo.west);
        \end{pgfonlayer}


    \end{tikzpicture}
    \vspace{-0.3cm}
    \caption{In this example tree, the subtree $\mathcal{B}_{k_1q}$ is highlighted in orange, $\mathcal{B}_{k_2q}$  in blue and $\mathcal{B}_{k_3q}$ in green. Leaf nodes are colored red. }
    %\vspace{-0.5cm}
    \label{fig:subtree}
\end{figure}

